Expressivity of bisimulation pseudometrics over analytic state spaces

A Markov decision process (MDP) is a state-based dynamical system capable of describing probabilistic behaviour with rewards. In this paper, we view MDPs as coalgebras living in the category of analytic spaces, a very general class of measurable spaces. Note that analytic spaces were already studied in the literature on labelled Markov processes and bisimulation relations. Our results are twofold. First, we define bisimulation pseudometrics over such coalgebras using the framework of fibrations. Second, we develop a quantitative modal logic for such coalgebras and prove a quantitative form of Hennessy-Milner theorem in this new setting stating that the bisimulation pseudometric corresponds to the logical distance induced by modal formulae.

==> fragments/app_otherTools.tex <==
\begin{lemma}
        \label{lem:fixPoint_ineq_approx}
    For a set $\spSet$ let\hbtodo{This can be removed since this is well known.} $ 
        L 
    $ be a set preordered by $\leq$ with $\emptyset \in L $ and
    $T \colon L \to L$ an order preserving function.
    Assume further that $ 
        l \coloneqq \lim_{i\to\infty} L^{\circ i} (\bot)(x, y) 
    $ exists.
    If for some $f \in L$ we have $ T(f) \leq l + \varepsilon $ for any $\varepsilon > 0$, then $
      l \leq f  
    $.
\end{lemma}

\begin{proof}
    Let $\mathrm{OP}$ denote the fact that $T$ is order preserving.
    The claim follows from the deduction
        \[
    \begin{prooftree}
        \hypo{\bot \leq f }
        \hypo{\mathrm{OP}}
        \infer2
            { \begin{multlined}[b]
                T^{\circ i}(\bot) 
                \leq T^{\circ i} (f)  
            \end{multlined}
            }
        \hypo{
                T({f })
            \leq f  + \varepsilon
        }
        \infer[double]1{T(f) \leq f }
        \hypo{\mathrm{OP}}
        \infer2
            {
                T^{\circ i} (f ) 
                \leq f  
            }
        \infer2
            {
                T^{\circ i} ( \bot ) \leq f  }
        \hypo
            { \begin{multlined}[b]
                    l(x,y) 
                 = \lim\limits_{i\to\infty} T^{\circ i} (\bot)(x, y)
            \end{multlined}}
        \infer2
            {l \leq f  }
    \end{prooftree}
    \]
    where all free $\varepsilon $ range over $(0,\infty)$, all free $i$ range over $\omega$ and all free $x,y$ range over $\spSet$.
\end{proof}

==> fragments/log-MDPs.tex <==
In this section, we will introduce a quantitative modal logic $\Sprache$ for MDPs and show its adequacy and expressivity w.r.t.\nolinebreak[3]\ the bisimulation pseudometric $\bdistance$ defined in the previous section as the least fixpoint of the functional $\gamma \circ \sigma^B$ (cf.\nolinebreak[3]\ \cref{cor:bdistance-exists}). Here the usage of `quantitative' is to signify that the semantics of a formula $\varphi\in\Sprache$ will be a real-valued predicate $\interpret{\varphi} \in \predicates \measSp$ over the state space of an MDP $\gamma \colon \measSp \to \BfunctorMDP \measSp$. Moreover, we follow \cite{CoalgModalLogicSurvey:2011} to state: the logic $\Sprache$\todo{Isn't adequacy rather a property of the interpretation than of the language?} is \definiendum{adequate} iff the bisimulation distance $\bdistance$ is below the logical distance $\ldistance = \sup_{\varphi\in\Sprache} \interpret{\varphi}^* d_E$ in the poset $\pred{\measSp \times \measSp}$, which in turn (recall that the poset of predicates is ordered by $\geq$) is equivalent to $\bdistance \geq \ldistance$, i.e.
\[
\forall_{x,x'\in X}\ \bdistance(x,x') \geq \ldistance (x,x') = \sup_{\varphi \in \Sprache} \interpret{\varphi}^*d_E (x,x') = \sup_{\varphi \in \Sprache} |\interpret{\varphi} (x) - \interpret{\varphi} (x')|.
\]
Here, $d_E$ is the Euclidean distance on the unit interval (i.e.\nolinebreak[3]\ $(r,s) \mapsto \abs{r-s}$). And we say that the logic $\Sprache$ is \definiendum{expressive} iff the converse of adequacy is true, i.e.\nolinebreak[3]\ $\bdistance \leq \ldistance$. Below we only considers logic for MDPs since the logical characterisation results for Markov processes can be derived by simply letting $\Sigma$ to be a singleton set.

==> fragments/prelim_cptPavings.tex <==
Properties of measurable spaces can conveniently characterised in terms of compact paving without having to invoke topologies.
A paving $\paving F$ on $\spSet$ is said to have the \definiendum{finite intersection property} (\definiendum{FIP}) is for any finite subset $ \paving F' \subseteq \paving F $ we have $\bigcap \paving F' \neq \emptyset$.
A paving is called $\cptPav$ is called \definiendum{countably compact} if for every countable subpaving $\paving S \subseteq \cptPav$ with FIP we have $\bigcap \paving S \neq \emptyset$.
In grasping this definition it may be useful to consider its contraposition as well: 
For any countable paving $\paving S \subseteq \cptPav$ with $\bigcap \paving S = \emptyset$ already $\bigcap F = \emptyset$ for some finite $\paving F \subseteq \paving S$. 
Also note that a topological space is countably compact if and only if the paving of its closed subsets is countably compact \cite[4A2A]{Fremlin}.

For perfectness we find that a measure space $\measdSp$ if \textit{perfect} if and only if for any countable paving $\paving S \subseteq \sAlg$ there is some $A \in \sAlg$ with $\meas(\complOp{A}) < \varepsilon$ such that $\paving S|_A$ is countably compact.
Moreover a measurable space $\measSp$ is \textit{smooth} if and only if there is a set $\spSet* \supseteq \spSet$ and a countably compact paving $\cptPav$ on $\spSet*$ such that $ \sAlg \subseteq \Souslin\cptPav $ \cite[1.1]{Falkner81}.

A measure on $\measSp$ is called \definiendum{countably compact} if it is inner regular with respect to some countably compact paving $\cptPav$, i.e.\nolinebreak[3]\ $ \meas(A) = \sup\setBuilder{ \meas(B) }{ B \in \sAlg \cap \cptPav } $ for every $A \in \sAlg$.
It is a remarkable feature of countable compactness that it is stable under push-forward \cite[452R]{Fremlin} (original result from \cite{Pachl79}).
In other word, the Giry monad restrict to a subfunctor assigning to each measurable space the collection of countably compact measures thereon.

Another remarkable property is that such measures admit disintegrations:
Given a consistent (i.e.\nolinebreak[3]\ $ f_* \meas = \meas* $) map $f\colon \measdSp \to \measdSp*$ of probability spaces a \definiendum{disintegration of $\meas $ over $\meas*$ consistent with $f$} is an $\spSet*$-indexed datum of \salg{}s $\sAlg_y$ and measures $\meas_y$ on $\sAlg_y$ such that for each $A \in \sAlg$ we have
\[
    \int \meas_y(A) \meas*(\diff y) = \meas(A)
\]
(implying of course that $\meas_y(A)$ is $\meas*$-almost surely defined for every $A \in \sAlg$).

\begin{lemma}
    Let $\measdSp$ be a countably compact measure space, $\measdSp*$ a $\sigma$-finite measure space, and $f \colon \spSet \to \spSet*$ an inverse-measure-preserving function. Then there is a disintegration $\{\meas_y\}_{y\in \spSet*}$ of $\meas$ over $\meas*$, consistent with $f$, such that $\meas_y (\spSet) \leqq 1$ for every $y \in \spSet*$. Moreover,
        \begin{enumerate}
            \item 
                if $\cptPav$ is a countably compact class of subsets of $\spSet$ such that $\meas$ is inner regular with respect to $\cptPav$, then we can arrange that $\cptPav \subseteq \operatorname{dom} \meas_y$ for every $y \in \spSet*$;
            \item 
                if, in (i), $\cptPav$ is closed under finite unions and countable intersections, then we can arrange that $\cptPav \subseteq \operatorname{dom} \meas_y$ and $\meas_y$ is inner regular with respect to $\cptPav$ for every $y \in \spSet*$.
        \end{enumerate}
\end{lemma}
\begin{proof}
    \Cite[452I]{Fremlin} (originally \cite{Pachl79}).
\end{proof}

